The Devil is in the Wrongly-classified Samples: Towards Unified Open-set Recognition

Open-set Recognition (OSR) aims to identify test samples whose classes are not seen during the training process. Recently, Unified Open-set Recognition (UOSR) has been proposed to reject not only unknown samples but also known but wrongly classified samples, which tends to be more practical in real-world applications. The UOSR draws little attention since it is proposed, but we find sometimes it is even more practical than OSR in the real world applications, as evaluation results of known but wrongly classified samples are also wrong like unknown samples. In this paper, we deeply analyze the UOSR task under different training and evaluation settings to shed light on this promising research direction. For this purpose, we first evaluate the UOSR performance of several OSR methods and show a significant finding that the UOSR performance consistently surpasses the OSR performance by a large margin for the same method. We show that the reason lies in the known but wrongly classified samples, as their uncertainty distribution is extremely close to unknown samples rather than known and correctly classified samples. Second, we analyze how the two training settings of OSR (i.e., pre-training and outlier exposure) influence the UOSR. We find although they are both beneficial for distinguishing known and correctly classified samples from unknown samples, pre-training is also helpful for identifying known but wrongly classified samples while outlier exposure is not. In addition to different training settings, we also formulate a new evaluation setting for UOSR which is called few-shot UOSR, where only one or five samples per unknown class are available during evaluation to help identify unknown samples. We propose FS-KNNS for the few-shot UOSR to achieve state-of-the-art performance under all settings.

==> tex/0_abstract.tex <==
\begin{abstract}
Open-set Recognition (OSR) aims to identify test samples whose classes are not seen during the training process.
%
Recently, Unified Open-set Recognition (UOSR) has been proposed to reject not only unknown samples but also known but wrongly classified samples,
%
which tends to be more practical in real-world applications.
%
%% The UOSR draws little attention since it is proposed, but we find sometimes it is even more practical than OSR in the real world applications, as evaluation results of known but wrongly classified samples are also wrong like unknown samples. 
%
In this paper, we deeply analyze the UOSR task under different training and evaluation settings to shed light on this promising research direction.
%% The related works of UOSR are rare as it is a newly proposed problem, so we deeply analyze the UOSR under different settings to shed light on this meaningful research direction.
%
For this purpose, we first evaluate the UOSR performance of several OSR methods and show a significant finding that the uncertainty distribution of almost all these methods is actually closer to the expectation of UOSR than OSR.
%
We show that the reason lies in the known but wrongly classified samples, as their uncertainty distribution is extremely close to unknown samples rather than known and correctly classified samples.
%
% \zsw{
% Second, we analyze the underlying rationale that how the two helpers of OSR, \emph{i.e.}, pre-training and outlier exposure, effect the UOSR.
% %
% }
Second, we analyze how the two training settings of OSR (\emph{i.e.}, pre-training and outlier exposure) influence the UOSR.
%
We find although they are both beneficial for distinguishing known and correctly classified samples from unknown samples, pre-training is also helpful for identifying known but wrongly classified samples while outlier exposure is not. 
%
In addition to different \emph{training settings}, we also formulate a new \emph{evaluation setting} for UOSR which is called few-shot UOSR, where only one or five samples per unknown class are available during evaluation to help identify unknown samples.
%
% Finally, we formulate the Few-shot Unified Open-set Recognition setting, where only one or five samples per unknown class are available during evaluation to help identify unknown samples. 
%
We propose FS-KNNS for the few-shot UOSR to achieve state-of-the-art performance under all settings.
%
% We propose a method named FS-KNNS, which does not require any additional operations and outlier data during training, but still achieves state-of-the-art performance under all settings.

\end{abstract}

==> tex/1_2_introduction.tex <==
\section{Introduction}

Neural networks have achieved tremendous success in the closed-set classification~\citep{deng2009imagenet}, where the test samples share the same In-Distribution (InD) class set with training samples. 
%
Open-Set Recognition (OSR)~\citep{towards_open} is proposed to tackle the challenge that some samples whose classes are not seen during training, which are Out-of-Distribution (OoD) data, may occur in the real world applications and should be rejected.
%
However, some researchers have argued that the model should not only reject OoD samples but also InD samples that are Wrongly classified (InW), as the model gives the wrong answers for both of them.
%
So Unified Open-set Recognition (UOSR) is proposed to only accept InD samples that are correctly classified (InC) and reject OoD and InW samples~\citep{kim2021unified} simultaneously.
%
The difference between the UOSR and OSR lies in the InW samples, where OSR is supposed to accept them while UOSR has the opposite purpose.
%
Actually, UOSR is more useful in most real-world applications, but it receives little attention from the research community as it has been proposed very recently and lacks comprehensive systematic research.
%
Therefore, we deeply analyze the UOSR problem in this work to fill this gap. 

We first apply existing OSR methods for UOSR in Sec.~\ref{sec:3}, and then analyze UOSR under different \textit{training settings} and \textit{evaluation settings} in Sec.~\ref{sec:4} and Sec.~\ref{sec:5} respectively.
%
In Sec.~\ref{sec:3}, several existing OSR methods are applied for UOSR, and we demonstrate a significant finding that \textit{the uncertainty distribution of almost all existing methods designed for OSR is actually closer to the expectation of UOSR than OSR}. 
%
In other words, simply changing the uncertainty ground truth of InW samples from 0 (OSR) to 1 (UOSR) can bring a very large performance gain, as shown in Fig.~\ref{fig:UOSR_OSR} (a). We show that this phenomenon holds for different network architectures, datasets, and domains (image and video recognition). We find the devil is in the InW samples that have similar uncertainty distribution with OoD samples rather than InC samples.

In Sec.~\ref{sec:4}, we introduce two \textit{training settings} into UOSR, including pre-training~\citep{hendrycks2019using} and outlier exposure~\citep{hendrycks2018deep,mcd,eb}, as they are both helpers of the OSR that introduce extra information beyond the training set.
%
Pre-training is to use the weights that are trained on a large-scale dataset for better down-task performance, and outlier exposure is to introduce some background data without labels into training to help the model classify InD and OoD samples. 
%
We find both of them have better performance for InC/OoD discrimination, which explains why they are beneficial for OSR. 
%
However, pre-training is also helpful for InC/InW discrimination, while outlier exposure has a comparable or even worse performance to distinguish InC and InW samples. 
%
The performance of UOSR can be regarded as the comprehensive results of InC/OoD and InC/InW discrimination so that both techniques can boost the performance of UOSR. 
%
We build up a comprehensive UOSR benchmark that involves both pre-training and outlier exposure settings, as shown in Fig.~\ref{fig:UOSR_OSR} (b).

In addition to the two aforementioned \textit{training settings}, 
% In addition to different training settings in Sec~\ref{sec:4}, 
%
we introduce a new \textit{evaluation setting} into UOSR in Sec.~\ref{sec:5}. 
%
We formulate the few-shot UOSR, similar to SSD~\citep{sehwag2021ssd} that proposes few-shot OSR, where 1 or 5 samples per OoD class are introduced for reference to better identify OoD samples. 
%
We first develop a KNN-based baseline ~\citep{sun2022out} FS-KNN for the few-shot UOSR. 
%
Although InC/OoD discrimination is improved due to the introduced OoD reference samples, the InC/InW discrimination is severely harmed compared to SoftMax baseline~\citep{hendrycks2016baseline}. 
%
To alleviate this problem, we propose FS-KNNS that dynamically fuses the FS-KNN with SoftMax uncertainty scores to keep high InC/InW and InC/OoD performance simultaneously. 
%
Our FS-KNNS achieves state-of-the-art performance under all settings in the UOSR benchmark, as shown in Fig.~\ref{fig:UOSR_OSR} (b), even without outlier exposure during training.
%
Note that InC/OoD performances are comparable between FS-KNNS and FS-KNN, but their distinct InC/InW performances makes FS-KNN better at OSR and FS-KNNS better at UOSR, which illustrates the difference between few-shot OSR and UOSR and the importance of InW samples during evaluation.

\begin{figure}
  \centering
  \includegraphics[width=0.99\linewidth]{iclr2023/figs/fig_1_r50_tiny_5.pdf}
  \vspace{-0.4cm}
  \caption{(a) shows that the UOSR performance is significantly better than OSR performance for the same method, which illustrates the uncertainty distribution of these OSR methods is actually closer to the
expectation of UOSR than OSR. 
%
(b) shows the UOSR performance under different settings and the skeleton of this paper. 
%
Results are based on the ResNet50 backbone. 
%
CIFAR100 and TinyImageNet are InD and OoD datasets, respectively.
%
(TS: Train from Scratch. TP: Train from Pre-training. OE: Outlier Exposure. FS: Few-shot.)
}
  \label{fig:UOSR_OSR}
  % \vspace{-0.6cm}
\end{figure}

==> tex/1_introduction.tex <==
\section{Introduction}

Neural networks have achieved tremendous success in the closed-set classification~\citep{deng2009imagenet}. However, in the real world applications, there is no guarantee that all test samples come from the classes included in the training set, referred to as In-Distribution (InD) classes. Therefore, rejecting samples whose classes are not seen during training, which are Out-of-Distribution (OoD) data, is significantly important. The corresponding task is called Open-Set Recognition (OSR)~\citep{towards_open}, which aims to correctly classify InD samples and reject OoD samples at the same time.

A rich line of OSR methods are developed for better open-set performance~\citep{hendrycks2016baseline,RPL,vaze2021open}. However, very recently some researchers argue that the model should not only reject OoD samples, but also reject InD samples that are Wrongly classified (InW), as the model gives the wrong answers for both of them. So Unified Open-set Recognition (UOSR) is proposed to only accept InD samples that are Correctly classified (InC), and reject both OoD and InW samples~\citep{xia2022augmenting, kim2021unified}. The difference between the UOSR and OSR lies in the InW samples, where OSR is supposed to accept them while UOSR has the opposite purpose.

We find the setting of UOSR is very useful and even more practical than OSR in the real world applications, as the evaluation results of InW samples are also wrong like OoD samples, so we should reject them rather than accept them. Therefore, we look deeper into the UOSR problem in this paper and hope to attract more researchers into this meaningful and new problem that has not received much attention. We begin from studying the UOSR performance of existing OSR methods, and we demonstrate a significant finding that \textit{almost all methods designed for OSR are actually more suitable for UOSR than OSR} in Sec.~\ref{sec:3}. In other words, simply changing the uncertainty ground truth of InW samples from 0 (OSR) to 1 (UOSR) can bring a very large performance gain, as shown in Fig.~\ref{fig:UOSR_OSR} (a). We show that this phenomenon holds for different network architectures, datasets and domains (image and video recognition). We find the devil is in the InW samples which have similar uncertainty distribution with OoD samples rather than InC samples.

In Sec.~\ref{sec:4}, to improve the UOSR performance of existing methods, we introduce two friends of OSR into UOSR, including pre-training~\citep{hendrycks2019using} and outlier exposure~\citep{hendrycks2018deep,mcd,eb}. Pre-training is to use the weights that are trained on a large scale dataset for better down-task performance, and outlier exposure is to introduce some background data without labels into training to help the model classify InD and OoD samples. We find both of them have better performance for InC/OoD discrimination, which explains why they are beneficial for OSR. However, pre-training is also helpful for InC/InW discrimination, while outlier exposure has the comparable or even worse performance to distinguish InC and InW samples. The performance of UOSR can be regarded as the comprehensive results of InC/OoD and InC/InW discrimination, so overall both techniques can boost the performance of UOSR. We build up a comprehensive UOSR benchmark which involves both pre-training and ourlier exposure settings, as shown in Fig.~\ref{fig:UOSR_OSR} (b).

In Sec.~\ref{sec:5}, we introduce the few-shot setting into UOSR to further improve the UOSR performance, similar with SSD~\citep{sehwag2021ssd} which proposes few-shot OSR. During evaluation, 5 or 1 samples per OoD class are introduced for reference to better identify OoD samples. We first develop a KNN based baseline ~\citep{sun2022out} FS-KNN to calculate the uncertainty based on the feature distance with InD samples and OoD reference samples. Although InC/OoD discrimination is improved due to the introduced OoD reference samples, the InC/InW discrimination is severely harmed compared to SoftMax baseline~\citep{hendrycks2016baseline}. To alleviate this problem, we propose FS-KNNS which dynamically fuses the FS-KNN with SoftMax uncertainty scores so that InC/InW performance is comparable with SoftMax while InC/OoD performance is largely improved because of FS-KNN. Our FS-KNNS achieves state-of-the-art performance under all settings in the UOSR benchmark, as shown in Fig.~\ref{fig:UOSR_OSR} (b), even without outlier exposure during training.

\begin{figure}
  \centering
  \includegraphics[width=0.99\linewidth]{iclr2023/figs/fig_1_r50_tiny_2.pdf}
  \vspace{-0.4cm}
  \caption{(a) shows that the UOSR performance is significantly better than OSR performance for the same method, which illustrates existing OSR methods are more suitable for the UOSR task. (b) shows the UOSR performance under different settings and the skeleton of this paper. (TS: Train from Scratch. TP: Train from Pre-training. OE: Outlier Exposure. FS: Few-shot.) Results are based on the ResNet50 backbone. CIFAR100 and TinyImageNet are InD and OoD datasets respectively. }
  \label{fig:UOSR_OSR}
  % \vspace{-0.6cm}
\end{figure}

==> tex/2_related.tex <==
\section{Towards Unified Open-set Recognition}

In this section, we first formalize the UOSR problem and then discuss the relation between UOSR and other uncertainty-related tasks, as the core of UOSR is also how to estimate better uncertainty scores to reject InW and OoD samples.

% In this section, we systematically introduce the different settings of all uncertainty-related tasks, including Selective Prediction (SP), Model Calibration (MC), Anomaly Detection (AD), Out-of-distribution Detection (OoDD), OSR, and UOSR. 
% %
% The comparison of these tasks is summarized in Table~\ref{tab:exp_set}. 
% %
% We first formalize the UOSR problem and then discuss the relation with other tasks.

\textbf{Unified Open-set Recognition.}
Suppose the training dataset is $
\mathcal{D}_\text{train} =
\{(\mathbf{x}_i, y_i)\}^{N}_{i=1}
\subset
\mathcal{X} \times \mathcal{C}
$, where $\mathcal{X}$ refers to the input space, \eg, images or videos, and $\mathcal{C}$ refers to the InD sets. In closed-set recognition, all test samples come from the InD sets, \ie, $
\mathcal{D}^{\text{closed}}_\text{test} = \{(\mathbf{x}_i, y_i)\}^{M}_{i=1}
\subset
\mathcal{X} \times \mathcal{C}
$. 
%
In OSR and UOSR, the test samples may come from OoD sets $\mathcal{U}$ which are not overlap with InD sets $\mathcal{C}$, so we have $
\mathcal{D}^{\text{open}}_\text{test}  = \mathcal{D}^{\text{closed}}_\text{test} \cup \mathcal{D}^{\text{unknown}}_\text{test} 
$, where $
\mathcal{D}^{\text{unknown}}_\text{test}  = \{(\mathbf{x}_i, y_i)\}^{M'}_{i=1}
\subset
\mathcal{X} \times \mathcal{U}
$. 
%
The InD test samples $\mathcal{D}^{\text{closed}}_\text{test}$ can be divided into two splits based on whether the sample is correctly classified or wrongly classified, \ie, $
\mathcal{D}^{\text{closed}}_\text{test}  = \mathcal{D}^{\text{closed-c}}_\text{test}  \cup \mathcal{D}^{\text{closed-w}}_\text{test} 
$, where $\mathcal{D}^{\text{closed-c}}_\text{test}  = \{(\mathbf{x}_i, y_i) | \hat{y}_i = y_i \}^{M}_{i=1}, \mathcal{D}^{\text{closed-w}}_\text{test}  = \{(\mathbf{x}_i, y_i) | \hat{y}_i \ne y_i \}^{M}_{i=1},$ and $\hat{y}_i$ refers to the model classification results of sample $\mathbf{x}_i$. 
%
The goal of UOSR is to reject InW and OoD samples and accept InC samples, so the ground truth uncertainty $u$ of $\mathcal{D}^{\text{closed-w}}_\text{test}$ and $\mathcal{D}^{\text{unknown}}_\text{test}$ is 1 while for $\mathcal{D}^{\text{closed-c}}_\text{test}$ it is 0, as shown in Table~\ref{tab:exp_set}.
%
The key of UOSR is how to estimate the uncertainty $\hat{u}$ to be close to the ground truth uncertainty $u$. 

\begin{wraptable}[9]{r}{0.48\textwidth}
\tablestyle{2pt}{1}
\vspace{-1.4em}
\caption{Comparison of uncertainty-related task settings. Cls: Classification. 0 and 1 refer to the corresponding ground truth uncertainty $u$, and $u$ is not fixed in MC.
}
\vspace{-1em}
\centering
\begin{tabular}{lccccc}
% \toprule[0.2pt]
\hline
&\textbf{InC} &  \textbf{InW} & \textbf{OoD} &\textbf{Ordinal Rank} & \textbf{InD Cls}\\
\hline
SP &0 & 1 & \xmark & \cmark & \cmark\\
AD &0 & 0 & 1 & \cmark & \xmark\\
OSR &0 & 0 & 1 & \cmark & \cmark\\
UOSR & 0 & 1 & 1 & \cmark & \cmark\\
MC &- & - & \xmark & \xmark & \cmark\\
\hline
% \bottomrule[0.2pt]
\end{tabular}
\label{tab:exp_set}
\vspace{-3em}
\end{wraptable}
The UOSR is proposed by~\citep{kim2021unified} very recently, so it has not attracted many researchers to this problem yet. 
%
SIRC~\citep{xia2022augmenting} augments SoftMax~\citep{hendrycks2016baseline} baseline for the better UOSR performance. 
%
% We look deeper into the UOSR problem in this paper and hope to draw more researchers' attention to this meaningful problem. 
%
Build upon these existing methods, we make a deep analysis of UOSR in this work.
%
In Table~\ref{tab:exp_set}, we compare different settings of the related uncertainty estimation tasks, and the detailed discussions are as follows.
% different settings of all uncertainty-related tasks, including Selective Prediction (SP), Model Calibration (MC), Anomaly Detection (AD), Out-of-distribution Detection (OoDD), OSR, and UOSR. 
% %
% The comparison of these tasks is summarized in Table~\ref{tab:exp_set}. 
%
% We first point out a significant finding but is dismissed before: the
% uncertainty distribution of almost all existing methods designed for OSR is actually closer to the expectation of UOSR than OSR (Sec.~\ref{sec:3}). 
% %
% Then we discuss how pre-training and outlier exposure affects UOSR performance (Sec.~\ref{sec:4}).
% %
% Finally, few-shot UOSR and a corresponding method FS-KNNS are proposed, and FS-KNNS achieves state-of-the-art performance under all settings (Sec.~\ref{sec:5}).

\textbf{Selective Prediction (SP).} 
%
Apart from the classical classification, SP also tries to estimate which sample is wrongly classified~\citep{tcp, crl, doctor}, so the ground truth uncertainty of InW is 1. 
%
SP is constrained under the closed-set scenario and does not consider OoD samples during evaluation, as shown in Table~\ref{tab:exp_set}, which is the key difference with UOSR.
%
We involve some SP methods in the UOSR benchmark in Sec.~\ref{sec:4}.

\textbf{Anomaly Detection (AD).} 
%
AD is to detect anomaly patches within an image or anomaly events within a video~\citep{deng2022anomaly, zaheer2022generative}. 
%
Therefore, AD is defined within a test sample, and there is no InD samples classification task. % (InD Cls in Table~\ref{tab:exp_set}). 
%
Unlike other tasks that assign uncertainty on the image or video level, AD assigns uncertainty on the pixel or frame level.

\textbf{Open-set Recognition (OSR) and Out-of-distribution Detection (OoDD).} 
%
The task settings of OSR and OoDD are same, but their datasets might be different. 
%
Both of them aim to accept all InD samples no matter they are InC or InW samples, and reject OoD samples. 
%
OSR divides one dataset into two splits and uses one of them as InD data to train the model, while another split is regarded as OoD samples~\citep{towards_open}. 
%
In contrast, OoDD uses a whole dataset as InD data and regards another dataset as OoD data~\citep{hendrycks2016baseline}. 
%
However, in the recent works about OSR in the video domain~\citep{bao2021evidential}, it utilizes the OoDD setting rather than the OSR setting. 
%
In this work, we use OSR to represent the task setting and use one dataset as InD data and another dataset as OoD data. 
%
As mentioned before, the distinction between UOSR and OSR is InW samples, where OSR aims to accept them, and UOSR aims to reject them, so the ground truth uncertainty of InW samples is 0 in OSR and 1 in UOSR, as shown in Table~\ref{tab:exp_set}. 
%
\textit{Better InC/OoD performance is beneficial for both UOSR and OSR, but higher InC/InW discrimination is preferred by UOSR but not wanted by OSR.}

\textbf{Model Calibration (MC).} 
%
All tasks mentioned above solve the uncertainty ordinal ranking problem, \ie, the ground truth uncertainty of each type of data is fixed, and the performance will be better if the estimated uncertainty is closer to the ground truth uncertainty~\citep{geifman2018bias}. 
%
In contrast, MC uses uncertainty to measure the probability of correctness~\citep{guo2017calibration}. 
%
For a perfect calibrated model, if we consider all samples with a confidence of 0.8, then 80\% of samples are correctly classified. 
%
In this case, 20\% InW samples with a confidence of 0.8 are perfect, but in other uncertainty-related tasks, InW samples are supposed to have a confidence of either 1 or 0. MC also does not consider OoD samples. 
%
See Appendix~\ref{app:a} for more relation between UOSR and MC.


==> tex/3_discussion_1.tex <==
\section{OSR Approaches for UOSR}



\label{sec:3}

\begin{table}[t]
\begin{minipage}[t]{0.48\textwidth}
\centering
\tablestyle{0.5pt}{1}
\caption{Uncertainty distribution analysis in image domain with ResNet50. OoD dataset: TinyImageNet. AUORC (\%) is reported.}
\vspace{-2mm}
\label{tab:U_OSR_image}
\begin{tabular}{lcccccccccccc}
\toprule[1pt]
\bf{Methods}  &\bf{InC/OoD} &\bf{InC/InW} &\bf{InW/OoD} &\bf{OSR} & \bf{UOSR} \\ \midrule
SoftMax   &84.69 &85.68 &50.64 &75.59 &84.90\\
ODIN &88.35 &80.76 &64.36 &81.65 &86.69\\
LC &84.60 &82.58 &55.14 &76.37 &84.16\\
OpenMax &85.16 &85.96 &51.27 &76.23 &85.33\\
OLTR &85.99 &85.74 &52.22 &77.10 &85.94\\
PROSER &87.04 &77.84 &62.57 &79.23 &84.82\\
\bottomrule[1pt]
\end{tabular}
\end{minipage}
\hspace{3mm}
\begin{minipage}[t]{0.48\textwidth}
\centering
\tablestyle{0.5pt}{1}
\caption{Uncertainty distribution analysis in video domain with TSM backbone. OoD dataset is HMDB51. AUORC (\%) is reported.}
\vspace{-2mm}
\label{tab:U_OSR_video}
\begin{tabular}{lcccccccccccc}
\toprule[1pt]
\bf{Methods}  &\bf{InC/OoD} &\bf{InC/InW} &\bf{InW/OoD} &\bf{OSR} & \bf{UOSR} \\ \midrule
OpenMax   &88.56 &82.53 &64.47 &82.27 &85.95\\
Dropout &85.36 &85.86 &48.92 &75.75 &85.58\\
BNN SVI &89.93 &88.85 &55.44 &80.10 &89.44\\
SoftMax &88.73 &88.01 &54.19 &79.72 &88.42\\
RPL &89.22 &88.06 &55.74 &79.67 &88.70\\
DEAR &89.33 &85.47 &56.78 &80.00 &87.56\\
\bottomrule[1pt]
\end{tabular}
\end{minipage}
\vspace{-4mm}
\end{table}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{iclr2023/figs/r50_tsm_fig2.pdf}
  \vspace{-0.4cm}
  \caption{(a) and (b) show the relation between UOSR and OSR performance in the image and video domain under ResNet50 and TSM backbones. 
  %
  Different color indicates different OoD datasets. 
  %
  The red-dotted diagonal is where UOSR has the same AUROC as OSR. 
  %
  Green arrows show the performance gap between UOSR and OSR for the same method.}
  \label{fig:UOSR_OSR_2}
  % \vspace{-0.6cm}
\end{figure}

In this section, we evaluate the existing OSR approaches for the UOSR problem, and show that the InW samples play a crucial role when evaluating the uncertainty quality.
% The difference between OSR and UOSR only lies in the uncertainty ground truth $u$ of InW samples, where $u=1$ for UOSR and $u=0$ for OSR, as shown in Table~\ref{tab:exp_set}. 
%
% However, we find that InW samples play a significant role when evaluating the uncertainty quality. 
%
Specifically, simply changing the ground truth uncertainty $u$ of InW samples from 0 to 1 can bring a large performance boost, as shown in Fig.~\ref{fig:UOSR_OSR_2}. 
%
Then we provide the comprehensive experiment results and discussion of this phenomenon.

\textbf{Applied Methods.} 
%
We reproduce several classical OSR methods and evaluate their UOSR and OSR performance in our experiments, including SoftMax~\citep{hendrycks2016baseline}, ODIN~\citep{ODIN}, LC~\citep{LC}, OpenMax~\citep{openmax}, OLTR~\citep{OLTR} and PROSER~\citep{PROSER} in the image domain, as well as DEAR~\citep{bao2021evidential}, RPL~\citep{RPL}, MC Dropout~\citep{dropout} and BNN SVI~\citep{BNNSVI} in the video domain.

\textbf{Datasets.}
%
In the image domain, the InD dataset is CIFAR100~\citep{CIFAR} and the OoD datasets are TinyImageNet~\citep{tinyimagenet} and LSUN~\citep{LSUN}. 
%
In the video domain, we follow~\citep{bao2021evidential} and adopt UCF101~\citep{ucf101} as InD dataset, while the OoD datasets are HMDB51~\citep{hmdb} and MiTv2~\citep{mitv2}.

\textbf{Experiments settings.} 
%
We train the network using the InD dataset and evaluate the UOSR and OSR performance based on the ground truth in Table~\ref{tab:exp_set}. 
%
The evaluation metric is AUORC~\citep{hendrycks2016baseline} which is a threshold-free value. 
%
The AUROC reflects the distinction quality of two uncertainty distributions. 
%
We adopt VGG13~\citep{VGG} and ResNet50~\citep{he2016deep} as the network backbone in the image domain and TSM~\citep{tsm} and I3D~\citep{i3d} in the video domain.
%
More experiment settings are in Appendix~\ref{app:b}.


\textbf{Results.} 
%
We provide the UOSR and OSR performance of different methods in Fig.~\ref{fig:UOSR_OSR_2}. 
%
It shows that all data points are above the red dotted diagonal, illustrating that the UOSR performance is significantly better than the OSR performance of the same method, and this relationship holds across different datasets, domains (image and video), and network architectures (See Appendix~\ref{app:uosr_osr} for results of more network backbones). 
%
The performance gap between UOSR and OSR of the same method can be very large, such as 8.84\% for OLTR when TinyImageNet is the OoD dataset, and 10.16\% for BNN SVI when the OoD dataset is MiTv2. 
%
Therefore, existing OSR methods have uncertainty distributions that are actually closer to the expectation of UOSR than OSR.

\textbf{Analysis.} 
%
To better understand our findings, we provide a detailed analysis of the uncertainty distribution relationships between InC, InW, and OoD samples in Tables~\ref{tab:U_OSR_image} and~\ref{tab:U_OSR_video}. 
%
Note that higher AUROC means a better distinction between two uncertainty distributions, and AUROC=50\% means two distributions overlap with each other. 
%
From Tables~\ref{tab:U_OSR_image} and~\ref{tab:U_OSR_video} we can clearly see that AUROC of InC/OoD and InC/InW are significantly higher than InW/OoD, and AUROC of InW/OoD is very close to 50\%. 
%
Therefore, the uncertainty distribution of InC samples is distinguishable from OoD and InW samples, and there is a lot of overlap between the uncertainty distributions of InW and OoD samples. 
%
We provide several uncertainty distribution visualizations in Fig.~\ref{fig:dis}, in which we can see that InW and OoD samples share a similar uncertainty distribution, while InC samples have smaller uncertainty in general. 
%
Therefore, the devil is in the InW samples for OSR, as InW samples have a similar uncertainty distribution to OoD samples rather than InC samples, which is contradictory to the ground truth of OSR. 
%
In contrast, the uncertainty distribution of InW samples is consistent with the expectation of UOSR, so existing OSR methods are actually more suitable for UOSR than OSR.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{iclr2023/figs/vgg_tsm.pdf}
  \vspace{-0.4cm}
  \caption{(a) and (b) are the SoftMax and ODIN methods in the image domain, while (c) and (d) are the SoftMax and DEAR methods in the video domain. OoD datasets are TinyImageNet for the image domain and HMDB51 for the video domain.}
  \label{fig:dis}
  % \vspace{-0.6cm}
\end{figure}

%
\textbf{Why?} 
%
We provide some empirical reasons for the finding that InW samples share a similar uncertainty distribution with OoD samples rather than InC samples. 
%
The model assigns low uncertainty for InC samples as they are well fitted by the model, and the cross-entropy loss encourages the SoftMax probability of the corresponding class to be close to 1.
%
However, InW and OoD samples are `hard' samples which are not well fitted by the model, so the cross-entropy loss cannot constrain the predictions to be confidence and their predictions tend to be more uncertain~\citep{vaze2021open, ranjan2017l2}. 
%
The fact that AUROC of InW/OoD is close to 50\% in Table~\ref{tab:U_OSR_image} and~\ref{tab:U_OSR_video} and the qualitative results in Fig.~\ref{fig:dis} can prove our claims.
%
% During the evaluation, some InD samples are wrongly classified due to the overfitting problem, so these InW samples are actually not well fitted by the model. 
% %
% Therefore, only InC samples are well fitted by the model, and both OoD and InW samples are not. 
% %
% This may give insight into why InW samples have a similar uncertainty distribution to OoD samples rather than InC samples.


\begin{wraptable}[8]{r}{0.48\textwidth}
\tablestyle{1pt}{1}
\vspace{-1.5em}
\caption{Relation between closed-set accuracy \textit{Acc.} (\%) and open-set performance. \textit{Aug:} Augmentation; \textit{Ep:} Epoch. AUROC (\%) is reported.
}
\vspace{-0.6em}
\centering
\begin{tabular}{ccccccc}
% \toprule[0.2pt]
\hline
\textbf{Aug.}&\textbf{Ep.} &\textbf{Acc.}&  \textbf{InC/OoD} & \textbf{InC/InW} &\textbf{OSR} & \textbf{UOSR}\\
\hline
\xmark &100 &59.41 & 81.65 & 82.47 & 68.64 & 81.89\\
\cmark &100 &68.83 & 84.18 & 85.13 & 73.71 & 84.40\\
\cmark &300 &73.28 & 84.69 & 85.68 & 75.59 & 84.90\\
\hline
% \bottomrule[0.2pt]
\end{tabular}
\label{tab:good_u}
\vspace{-3em}
\end{wraptable}
\textbf{A better closed-set model is better for UOSR.} 
% 分析太浅
Recently, \citep{vaze2021open} found that better closed-set performance means better OSR performance. 
%
We provide a deeper explanation of this finding and show that this conclusion also holds for UOSR. 
%
Table~\ref{tab:good_u} shows that we improve the closed-set accuracy through data augmentation and longer training~\citep{vaze2021open}. 
%
The open-set method is the SoftMax baseline with ResNet50 backbone, and the OoD dataset is TinyImageNet. 
%
For OSR, we can see that AUROC of InC/OoD is significantly better than OSR, which indicates the uncertainty distribution of InW samples are contradictory with the expectation of OSR. So less InW samples and better InC/OoD performance are two reasons for better OSR performance when closed-set accuracy is higher.
%
For UOSR, both the InC/InW and InC/OoD performance are improving with the growth of closed-set accuracy, which brings better UOSR performance. 

==> tex/4_discussion_2.tex <==
\section{Pre-training and Outlier Exposure}
\label{sec:4}

After directly applying existing OSR methods for UOSR in Sec.~\ref{sec:3}, we explore two additional training settings in this section, including pre-training~\citep{hendrycks2019using} and outlier exposure~\citep{hendrycks2018deep}, which are effective methods to improve the OSR performance because of introduced extra information beyond the training set. 
%
Pre-training is to use large-scale pre-trained weights for initialization for better down-task performance. 
%
Outlier exposure is to introduce some unlabeled outlier data (OD) during training and regard these outlier data as the proxy as OoD data to improve the open-set performance. 
%
We find both of them also have a positive effect on UOSR, but for different reasons.

\textbf{Pre-training settings.} In the image domain, we use BiT pre-training weights~\citep{bit} for ResNet50 and ImageNet~\citep{deng2009imagenet} pre-training weights for VGG13. In the video domain, Kinetics400~\citep{i3d} pre-trained weights are used for initialization.

\textbf{Outlier exposure settings.} In the image domain, we use 300K Random Images dataset~\citep{hendrycks2018deep} as outlier data. In the video domain, outlier data comes from Kinetics400, and we filter out the overlapping classes with InD and OoD datasets. We implement several outlier exposure based methods, including OE~\citep{hendrycks2018deep}, EB~\citep{eb}, Energy~\citep{energy}, VOS~\citep{vos} and MCD~\citep{mcd}.

\begin{table}[t]
\centering
\tablestyle{3pt}{0.5}
\caption{UOSR benchmark in the image domain under the ResNet50 model. InD dataset is CIFAR100 while the OoD dataset is TinyImageNet. ${\dagger}, {\ddagger}, {\Diamond}$ refer to OSR-based, SP-based, UOSR-based methods. OD: Outlier Data. AUORC (\%), AURC ($\times10^3$) and Acc. (\%) are reported.}
\vspace{-3mm}
\label{tab:bench_r50}
\begin{tabular}{lccccccccccccc}
\toprule[1pt]
&& \multicolumn{4}{c}{\bf{w/o pre-training}} &\multicolumn{4}{c}{\bf{w/ pre-training}} \\ 
\cmidrule(r){3-6}\cmidrule(r){7-10} && \multicolumn{3}{c}{\bf{UOSR}} &\bf{OSR} &\multicolumn{3}{c}{\bf{UOSR}} &\bf{OSR} \\
\cmidrule(r){3-5} \cmidrule(r){6-6} \cmidrule(r){7-9} \cmidrule(r){10-10} 
\bf{Methods} &\bf{OD} &\bf{Acc.$\uparrow$}  &\bf{AURC$\downarrow$}   & \bf{AUROC$\uparrow$}   & \bf{AUROC$\uparrow$}   &\bf{Acc.$\uparrow$} &\bf{AURC$\downarrow$}   & \bf{AUROC$\uparrow$}   & \bf{AUROC$\uparrow$}\\ \midrule
SoftMax$^{\dagger}$ &\xmark&73.28 &363.55 &84.90 &75.59 &86.44 &260.14 &90.50 &85.93   \\
ODIN$^{\dagger}$    &\xmark&72.08 &371.92  &86.69 &81.65 &86.48 &261.42 &91.81 &91.47\\
LC$^{\dagger}$     &\xmark&72.08 &372.55 &84.16 &76.37 &86.48 &280.69 &87.68 &85.16\\
OpenMax$^{\dagger}$ &\xmark&73.64 &361.22 &85.33 &76.23 &86.43 &261.53 &90.29 &85.86\\
OLTR$^{\dagger}$  &\xmark&73.69 &357.79 &85.94 &77.10 &86.22 &260.17 &90.59 &86.05\\
PROSER$^{\dagger}$ &\xmark&68.08 &394.48 &84.82 &79.23  &81.32 &301.78 &90.20 &89.29\\ \midrule
BCE$^{\ddagger}$ &\xmark&73.29 &369.91  &84.29 &74.59 &86.39 &257.74 &90.79  &86.50   \\
TCP$^{\ddagger}$ &\xmark&71.80 &369.17 &85.17 &75.46 &86.83 &261.97 &89.95 &85.67\\
DOCTOR$^{\ddagger}$ &\xmark &72.08 &378.45 &84.48 &75.06 &86.48 &262.05 &90.24 &85.75\\ \midrule
SIRC(MSP, $\left \| z \right \| _1$)$^{\Diamond}$ &\xmark&73.13 &358.93 &85.77 &76.67 &86.44 &260.08 &90.53 &85.98\\
SIRC(MSP, Res.)$^{\Diamond}$ &\xmark&73.13 &348.40 &87.26 &80.29 &86.44 &247.75 &92.99 &90.39\\
SIRC($-\mathcal{H}$, $\left \| z \right \| _1$)$^{\Diamond}$ &\xmark&73.13 &355.62 &86.57 &78.16 &86.44 &257.28 &91.23 &87.27\\
SIRC($-\mathcal{H}$, Res.)$^{\Diamond}$ &\xmark&73.13 &346.21 &87.71 &81.43 &86.44 &244.55  &93.68 &91.62\\ 
\midrule
OE &\cmark&73.54 &339.59 &88.78 &84.35 &85.43 &255.77 &92.54 &90.65\\
EB &\cmark&71.82 &366.65  &86.06 &81.95 &85.06 &269.79 &90.84 &90.38\\
Energy &\cmark&73.10 &349.56 &87.34 &79.34 &84.66 &269.74 &90.98 &87.09\\
VOS &\cmark&73.18 &331.12 &89.96 &85.78 &85.93 &251.44 &92.92 &91.34\\
MCD &\cmark&70.88 &365.82 &86.97 &79.88  &81.96 &287.21 &90.43 &86.59\\
\bottomrule[1pt]
\end{tabular}
\end{table}

\textbf{UOSR benchmark settings.} We include OSR-based, SP-based, and UOSR-based methods to build a comprehensive UOSR benchmark. 
%
%%The OSR-based methods are already listed in Sec.~\ref{sec:3}. 
%
We implement several Selective Prediction (SP) based methods, including BCE, TCP~\citep{tcp}, CRL~\citep{crl}, and DOCTOR~\citep{doctor}. Although these SP methods are originally designed to differentiate InC and InW samples, we adopt them in the UOSR setting to build a more comprehensive benchmark. The only UOSR-based method is SIRC~\citep{xia2022augmenting}, which combines two uncertainty scores for better UOSR performance. The evaluation metrics are AURC and AUROC~\citep{kim2021unified}. More details can be found in Appendix~\ref{app:b}.

\begin{table}[t]
\centering
\tablestyle{3pt}{0.5}
\caption{UOSR benchmark in the video domain under the TSM model. InD dataset is UCF101 while the OoD dataset is HMDB51. ${\dagger}, {\ddagger}, {\Diamond}$ refer to OSR-based, SP-based, UOSR-based methods. OD: Outlier Data. AUORC (\%), AURC ($\times10^3$) and Acc. (\%) are reported.}
\vspace{-3mm}
\label{tab:bench_tsm}
\begin{tabular}{lccccccccccccc}
\toprule[1pt]
&& \multicolumn{4}{c}{\bf{w/o pre-training}} &\multicolumn{4}{c}{\bf{w/ pre-training}} \\ 
\cmidrule(r){3-6}\cmidrule(r){7-10} && \multicolumn{3}{c}{\bf{UOSR}} &\bf{OSR} &\multicolumn{3}{c}{\bf{UOSR}} &\bf{OSR} \\
\cmidrule(r){3-5} \cmidrule(r){6-6} \cmidrule(r){7-9} \cmidrule(r){10-10} 
\bf{Methods} &\bf{OD} &\bf{Acc.$\uparrow$}  &\bf{AURC$\downarrow$}   & \bf{AUROC$\uparrow$}   & \bf{AUROC$\uparrow$}   &\bf{Acc.$\uparrow$} &\bf{AURC$\downarrow$}   & \bf{AUROC$\uparrow$}   & \bf{AUROC$\uparrow$}\\ \midrule
OpenMax$^{\dagger}$  &\xmark     & 73.92   & 185.81 & 85.95  &82.27               & 95.32   & 75.75  &91.22   &90.89        \\
MC Dropout$^{\dagger}$ &\xmark   & 73.63  & 184.66   & 85.58 &75.75           & 95.06   & 79.53    &90.30 &88.23     \\
BNN SVI$^{\dagger}$   &\xmark  & 71.51  & 181.45   & 89.44  &80.10          & 94.71   & 69.89    &93.58  &91.81  \\
SoftMax$^{\dagger}$ &\xmark  & 73.92  & 173.14   & 88.42  &79.72          & 95.03   & 68.08  &93.94 &91.75 \\
RPL$^{\dagger}$ &\xmark & 71.46  & 186.18   & 88.70  &79.67          & 95.59   & 72.88 &92.44 &90.53          \\
DEAR$^{\dagger}$  &\xmark  & 71.33 & 215.80     &  87.56  &80.00           & 94.41   & 102.01    &91.50   &91.49     \\
\midrule
BCE$^{\ddagger}$ &\xmark&69.90 &223.57 &83.27 &78.96 &93.66 &110.42 &83.83 &81.64\\
CRL$^{\ddagger}$ &\xmark&71.80 &183.76&88.75&78.57 &95.22 &67.61 &93.36  &91.38\\
DOCTOR$^{\ddagger}$ &\xmark&72.01 &182.04&88.73 &79.76 &95.06 &65.61 &93.89 &91.80\\ \midrule
SIRC(MSP, $\left \| z \right \| _1$)$^{\Diamond}$ &\xmark&73.59    & 173.32 &   88.71 &80.33 &95.00 &65.97 &93.74 &91.42\\
SIRC(MSP, Res.)$^{\Diamond}$ &\xmark&73.59   & 174.76 &88.17 &78.74 &95.00 &65.43 &93.83  &91.73\\
SIRC($-\mathcal{H}$, $\left \| z \right \| _1$)$^{\Diamond}$ &\xmark&73.59   & 172.30 &   89.27 &81.61 &95.00 &66.11 &94.06 &91.95\\
SIRC($-\mathcal{H}$, Res.)$^{\Diamond}$ &\xmark&73.59    & 175.79 &   88.50  &79.62 &95.00 &69.06 &94.07 &92.18\\
\midrule
OE &\cmark&       74.42                & 162.36  &   90.19 &86.29 &94.71 &67.93 &94.33  &93.40\\
EB &\cmark&       70.90                & 212.01  &   85.32 &86.47 &94.66 &67.83 &94.40 &93.06\\
Energy &\cmark&       74.00         & 187.82 &   86.10 &84.51&95.27 &65.68 &94.44 &93.62 \\
VOS &\cmark&       74.68               & 172.71 &   87.98 &87.09 &94.79 &64.99 &94.97&93.72   \\
MCD &\cmark&       72.49               & 168.83 &   91.26 &85.57 &93.47 &71.19 &95.34 &93.68\\
\bottomrule[1pt]
\end{tabular}
\end{table}

\textbf{Results.} 
%
The UOSR benchmarks for image and video domains are Table~\ref{tab:bench_r50} and~\ref{tab:bench_tsm} respectively. 
%
See Appendix~\ref{app:uosr_vgg_bench} for the results of different model architectures. 
%
First, we can see the AUROC of UOSR is higher than OSR for almost all the methods under both settings, \ie, pre-training and outlier exposure, which further strengthens the conclusion that the uncertainty distribution of OSR methods is closer to the ground truth of UOSR. For instance, AUROC is 87.34 for UOSR and 79.34 for OSR under the Energy method w/o pre-training in Table~\ref{tab:bench_r50}.
%
Second, pre-training and outlier exposure can effectively boost the UOSR and OSR performance
%
, \eg, the pre-training boost the AUROC of UOSR/OSR from 84.90/75.59 to 90.50/85.93 for the SoftMax, and outlier exposure method VOS has 89.96/85.78 AUROC of UOSR/OSR compared to 84.90/75.59 of SoftMax in Table~\ref{tab:bench_r50}.

\textbf{Analysis.} 
%
To better understand why pre-training and outlier exposure are helpful for UOSR and OSR, we provide the InC/InW and InC/OoD discrimination performance of each method in Fig.~\ref{fig:ablation}. 
%
We can see that almost all outlier exposure methods are in the Q2, which means that outlier exposure methods have lower InC/InW AUROC and higher InC/OoD AUROC than the SoftMax baseline. 
%
For OSR, both lower InC/InW and higher InC/OoD AUROC are beneficial, but only higher InC/OoD AUROC is wanted for UOSR, while lower InC/InW AUROC is not. This can explain why some of the UOSR performances with outlier exposure are comparable or even worse than the baseline, such as EB, Energy, and VOS in the video domain Table~\ref{tab:bench_r50}, but all of the OSR performances are increased. In contrast, pre-training is helpful for both InC/InW and InC/OoD AUROC, as methods with pre-training are in the Q1. Therefore, outlier exposure and pre-training bring the UOSR performance gain for different reasons. InC/OoD performance is improved by both of the techniques, but pre-training is also helpful for InC/InW, but outlier exposure is not. This can be explained by the fact that the model may see additional InD samples during pre-training so that the closed-set accuracy and InC/InW discrimination are improved. In contrast, outlier exposure only provides OoD data but no more InD data, so only InC/OoD performance is improved.


==> tex/5_few-shot.tex <==
\section{Few-shot Unified Open-set Recognition}
\label{sec:5}
\begin{figure}[t]
\vspace{-0.4cm}
  \centering
  \includegraphics[width=0.99\linewidth]{iclr2023/figs/ablation_r50_tsm.pdf}
  \vspace{-0.5cm}
  \caption{(a) and (b) plot the InC/InW and InC/OoD discrimination in the image and video domain. We set the SoftMax method training from scratch as the original point and divide the coordinate system into 4 quadrants (Q1 to Q4).}
  \label{fig:ablation}
  \vspace{-0.3cm}
\end{figure}

In addition to the analysis of two useful training settings in Sec.~\ref{sec:4}, we introduce a new evaluation setting into UOSR in this section. Inspired by the recent work SSD~\citep{sehwag2021ssd} which proposes the few-shot OSR, we introduce the few-shot UOSR, where 1 or 5 samples per OoD class can be introduced for reference to better distinguish OoD samples. The introduced reference OoD datasets are marked as $\mathcal{D}_{test}^{ref} = \{(\mathbf{x}_i, y_i)\}^{N'}_{i=1}
\subset
\mathcal{X} \times \mathcal{U}$. We show that few-shot UOSR has distinct challenges from few-shot OSR because of InW samples, and we propose our FS-KNNS method to achieves the state-of-the-art UOSR performance even without outlier exposure during training.
\begin{table}[t]
\centering
\tablestyle{1pt}{0.5}
\caption{Results of few-shot UOSR in the image domain. Model is ResNet50 with pre-training. InD and OoD datasets are CIFAR100 and TinyImageNet. AUORC (\%) and AURC ($\times10^3$) are reported.}
\vspace{-3mm}
\label{tab:fs_r50}
\begin{tabular}{lccccccccccccccc}
\toprule[1pt]
&\multicolumn{5}{c}{\bf{5-shot}} &\multicolumn{5}{c}{\bf{1-shot}}\\ \cmidrule(r){2-6} \cmidrule(r){7-11}
&\bf{AURC$\downarrow$} &  \multicolumn{4}{c}{\bf{AUROC$\uparrow$}} &\bf{AURC$\downarrow$} &  \multicolumn{4}{c}{\bf{AUROC$\uparrow$}}\\ \cmidrule(r){2-2} \cmidrule(r){3-6} \cmidrule(r){7-7} \cmidrule(r){8-11}
\bf{Methods}  &\cellcolor{gray_2}\bf{UOSR} &\cellcolor{gray_2}\bf{UOSR} & \bf{OSR} &\bf{InC/OoD} &\bf{InC/InW} &\cellcolor{gray_2}\bf{UOSR} &\cellcolor{gray_2}\bf{UOSR} & \bf{OSR} &\bf{InC/OoD} &\bf{InC/InW}\\ \midrule
SoftMax   &\cellcolor{gray_2}260.14  &\cellcolor{gray_2}90.51 &85.93 &90.64 &89.58 &\cellcolor{gray_2}260.14  &\cellcolor{gray_2}90.51 &85.93 &90.64 &89.58\\
KNN  &\cellcolor{gray_2}245.48 &\cellcolor{gray_2}93.45 &92.34 &94.86 &83.08 &\cellcolor{gray_2}245.48 &\cellcolor{gray_2}93.45 &92.34 &94.86 &83.08\\ \midrule
FS-KNN &\cellcolor{gray_2}238.54 &\cellcolor{gray_2}95.09 &95.91 &97.20 &79.58 &\cellcolor{gray_2}239.71 &\cellcolor{gray_2}94.67 &94.91 &96.52 &81.04\\
SSD &\cellcolor{gray_2}246.42 &\cellcolor{gray_2}94.95 &\bf{97.89} &\bf{98.32} &70.14 &\cellcolor{gray_2}245.99 &\cellcolor{gray_2}94.16 &\bf{96.51} &\bf{97.16} &72.09 \\ \midrule
FS-KNN+S &\cellcolor{gray_2}239.49 &\cellcolor{gray_2}94.14 &91.64 &95.27 &85.85 &\cellcolor{gray_2}240.30 &\cellcolor{gray_2}93.97 &91.36 &94.99 &86.45 \\
FS-KNN*S &\cellcolor{gray_2}255.82 &\cellcolor{gray_2}91.26 &87.10 &91.47 &\textbf{89.67} &\cellcolor{gray_2}255.69 &\cellcolor{gray_2}91.30 &87.16 &91.51 &\textbf{89.69} \\
SIRC &\cellcolor{gray_2}241.58 &\cellcolor{gray_2}93.85 &91.42 &94.44 &89.58 &\cellcolor{gray_2}239.64 &\cellcolor{gray_2}94.20 &92.03 &94.87 &89.26 \\ \midrule
FS-KNNS &\cellcolor{gray_2}\bf{231.61} &\cellcolor{gray_2}\bf{95.51} &94.16 &96.54 &87.98 &\cellcolor{gray_2}\bf{234.84} &\cellcolor{gray_2}\bf{94.91} &93.10 &95.84 &88.08\\
\bottomrule[1pt]
\end{tabular}
\end{table}
\begin{figure}[t]
  \centering
  \includegraphics[width=0.99\linewidth]{iclr2023/figs/fs-knns-image.pdf}
  \vspace{-0.4cm}
  \caption{Uncertainty scores of each test sample (a) and uncertainty distribution of SoftMax (b), FS-KNN (c), and FS-KNNS (d).}
  \label{fig:fs_image}
  % \vspace{-0.6cm}
\end{figure}
\textbf{Baselines and dataset settings.} SSD is the only existing few-shot OSR method that utilizes the Mahalanobis distance with InD training samples $\mathcal{D}_{train}$ and OoD reference samples $\mathcal{D}_{test}^{ref}$. KNN~\citep{sun2022out} utilizes the feature distance with samples in $\mathcal{D}_{train}$ as uncertainty scores and shows it is better than Mahalanobis distance. So we slightly modify KNN to adapt to the few-shot UOSR and find the modified FS-KNN can already beat SSD. $\mathcal{D}_{test}^{ref}$ comes from the validation set of TinyImageNet and training set of UCF101 in the image and video domain. We repeat the evaluation process until all OoD reference samples are used and calculate the mean as the final few-shot result.

% \textbf{KNN.} We begin with the uncertainty calculation of KNN. Given a test sample $\mathbf{x}^*$ and a feature extractor $f$, the feature representation of $\mathbf{x}^*$ is $\mathbf{z}^*=f(\mathbf{x}^*)$. We then store the feature representation of the training set $\mathcal{Z}_{train} = (\mathbf{z}_1, \mathbf{z}_2, ..., \mathbf{z}_N)$, where $\mathbf{z}_i=f(\mathbf{x}_i), \mathbf{x}_i \in \mathcal{D}_{train}$. Then the cosine similarity between the test sample $\mathbf{x}^*$ and each training sample $\mathbf{x}_i$ is calculated and denoted as $\mathcal{S}_{train} = (d_1, d_2, ..., d_N)$, where $d_i = (\mathbf{z}^*\cdot \mathbf{z}_i)/(\left \| \mathbf{z}^* \right \| \cdot \left \| \mathbf{z}_i \right \| ), \mathbf{z}_i \in \mathcal{Z}_{train}$. The idea of KNN is that the uncertainty is supposed to be lower if the test sample is more similar to training samples. The uncertainty score is calculated as Eq.~\ref{eq:knn}, where $topK$ means the $K^{th}$ largest value:
% \begin{equation}
%     \hat{u}_{knn} = 1 - topK(S_{train}).
%     \label{eq:knn}
% \end{equation}
\textbf{FS-KNN.} Given a test sample $\mathbf{x}^*$ and a feature extractor $f$, the feature of $\mathbf{x}^*$ is $\mathbf{z}^*=f(\mathbf{x}^*)$. The cosine similarity set between $\mathbf{z}^*$ and the feature set of $\mathcal{D}_{train}$ is $\mathcal{S}_{train} = \{{d}_i\}^{N}_{i=1}, d_i = (\mathbf{z}^*\cdot \mathbf{z}_i)/(\left \| \mathbf{z}^* \right \| \cdot \left \| \mathbf{z}_i \right \| ), \mathbf{z}_i = f(\mathbf{x}_i), \mathbf{x}_i \in \mathcal{D}_{train}$. $\mathcal{S}_{test}^{ref}$ is similar with $\mathcal{S}_{train}$ except $\mathbf{x}_i$ comes from $\mathcal{D}_{test}^{ref}$. We believe the uncertainty should be higher if the test sample is more similar to reference OoD samples and not similar with InD samples. Therefore, the uncertainty score is
\vspace{-0.15cm}
\begin{equation}
    \hat{u}_{fs-knn} = 1 - topK(S_{train}) + topK(S_{test}^{ref}),
    \vspace{-0.15cm}
\end{equation}
% \begin{table}[t]
% \centering
% \tablestyle{1pt}{0.5}
% \caption{Results of few-shot UOSR in the image domain. Model is ResNet50 with pre-training. InD and OoD datasets are CIFAR100 and TinyImageNet.}
% \vspace{-3mm}
% \label{tab:fs_r50}
% \begin{tabular}{lccccccccccccccc}
% \toprule[1pt]
% &\multicolumn{5}{c}{\bf{5-shot}} &\multicolumn{5}{c}{\bf{1-shot}}\\ \cmidrule(r){2-6} \cmidrule(r){7-11}
% &\bf{AURC$\downarrow$} &  \multicolumn{4}{c}{\bf{AUROC$\uparrow$}} &\bf{AURC$\downarrow$} &  \multicolumn{4}{c}{\bf{AUROC$\uparrow$}}\\ \cmidrule(r){2-2} \cmidrule(r){3-6} \cmidrule(r){7-7} \cmidrule(r){8-11}
% \bf{Methods}  &\bf{UOSR} &\bf{UOSR} & \bf{OSR} &\bf{InC/OoD} &\bf{InC/InW} &\bf{UOSR} &\bf{UOSR} & \bf{OSR} &\bf{InC/OoD} &\bf{InC/InW}\\ \midrule
% SoftMax   &260.14  &90.51 &85.93 &90.64 &89.58 &260.14  &90.51 &85.93 &90.64 &89.58\\
% KNN  &245.48 &93.45 &92.34 &94.86 &83.08 &245.48 &93.45 &92.34 &94.86 &83.08\\ \midrule
% FS-KNN &238.55 &95.09 &95.91 &97.20 &79.58 &239.71 &94.67 &94.91 &96.52 &81.04\\
% SSD &246.42 &94.95 &\bf{97.89} &\bf{98.32} &70.14 &245.99 &94.16 &\bf{96.51} &\bf{97.16} &72.09 \\ \midrule
% FS-KNN+S &239.49 &94.14 &91.64 &95.27 &85.85 &240.30 &93.97 &91.36 &94.99 &86.45 \\
% FS-KNN*S &255.82 &91.26 &87.10 &91.47 &\textbf{89.67} &255.69 &91.30 &87.16 &91.51 &\textbf{89.69} \\
% SIRC &241.58 &93.85 &91.42 &94.44 &89.58 &239.64 &94.20 &92.03 &94.87 &89.26 \\ \midrule
% FS-KNNS &\bf{231.61} &\bf{95.51} &94.16 &96.54 &87.98 &\bf{234.84} &\bf{94.91} &93.10 &95.84 &88.08\\
% \bottomrule[1pt]
% \end{tabular}
% % \end{table}
where $topK$ means the $K^{th}$ largest value. The performances of SoftMax, KNN, FS-KNN, and SSD are in Table~\ref{tab:fs_r50} and~\ref{tab:fs_video}. Pre-training is used for better performance. FS-KNN has better InC/OoD performance than KNN as reference OoD samples are introduced. Although the overall UOSR performance of FS-KNN is better than the SoftMax baseline, \textit{the InC/InW performance is significantly sacrificed, which is also an important aspect of UOSR.} For example, InC/InW performance drops from 89.58 to 79.58 in the 5-shot results of Table~\ref{tab:fs_r50}. So we naturally ask a question: \textit{Can we improve the InC/OoD performance based on the introduced OoD reference samples while keeping similar InC/InW performance with SoftMax baseline?} This is the key difference between few-shot OSR and few-shot UOSR, as low InC/InW performance is wanted in OSR but not preferred in UOSR.

\textbf{FS-KNNS.} Inspired by SIRC~\citep{xia2022augmenting}, we aim to find a way to fuse SoftMax and FS-KNN scores so that the mixed score can keep the high InC/OoD performance of FS-KNN and meanwhile has the comparable InC/InW performance with SoftMax. The uncertainty distributions of SoftMax and FS-KNNS are depicted in Fig.~\ref{fig:fs_image}. We find that OoD samples have larger uncertainty than InW and InC samples in the FS-KNN method, but the uncertainty of InC samples overlaps a lot with InW samples, which explains the reason that InC/OoD performance is high but InC/InW performance is low. In contrast, InW and OoD samples share similar uncertainty in the SoftMax method, which brings higher InC/InW performance. Therefore, we want to keep the uncertainty of InW samples in the SoftMax method, as well as the uncertainty of OoD samples in the FS-KNN method. In this way, the mixed scores obtain the high InC/OoD performance from FS-KNN while keeping the comparable InC/InW performance of SoftMax. We call this method FS-KNN with SoftMax (FS-KNNS), and the uncertainty is
\vspace{-0.2cm}
\begin{equation}
    \hat{u}_{fs-knns} = u_{0} + \frac{1}{1+\ve^{-\alpha (u_{1}-\lambda_{knns})}}u_1,
    \label{eq:knns}
    \vspace{-0.15cm}
\end{equation}
where $u_0$ and $u_1$ refer to the uncertainty score of SoftMax and FS-KNN, respectively. $\lambda_{knns}$ is a threshold to determine when the weight of $u_1$ becomes large, and $\alpha$ is a coefficient to control the change rate of the weight. $\hat{u}_{fs-knns}$ will be largely influenced by $u_1$ when $u_1>\lambda_{knns}$. A proper $\lambda_{knns}$ should be located between the InW and OoD samples, as shown in Fig.~\ref{fig:fs_image} (a) and (c). In this way, the uncertainty of InW samples is mainly controlled by SoftMax, and OoD samples are strengthened by FS-KNN. Ablation study about hyperparameters $K, \alpha, \text{and } \lambda_{knns}$ is in Appendix~\ref{app:ablation_fs}.
% \begin{wrapfigure}[15]{r}{0.48\textwidth}
% \centering
% \includegraphics[width=1\linewidth]{iclr2023/figs/all_video.pdf}
% \vspace{-9mm}
% \caption{UOSR performance under all settings in the video domain.
% }
% \label{fig:all_video}
% % \vspace{-3em}
% \end{wrapfigure}

\begin{wrapfigure}[15]{r}{0.45\textwidth}
\vspace{-0.5cm}
\centering
  \includegraphics[width=0.99\linewidth]{iclr2023/figs/all_video.pdf}
  \vspace{-0.8cm}
  \caption{UOSR performance under all settings of TSM backbone in the video domain. OoD dataset is HMDB51.}
  \label{fig:all_video}
\end{wrapfigure}
\textbf{Discussion.} The uncertainty distribution of FS-KNNS is shown in Fig.~\ref{fig:fs_image} (d), which shows the uncertainty of InC and InW samples are similar to SoftMax (b), but the uncertainty of OoD samples is larger. From Table~\ref{tab:fs_r50} and~\ref{tab:fs_video}, we can see our FS-KNNS has significantly better InC/InW performance than FS-KNN (87.98 and 79.58 under ResNet50), and meanwhile keeps the high InC/OoD performance, so the overall UOSR performance is better than both SoftMax and FS-KNN. We also try three score fusion methods, including FS-KNN+S, FS-KNN*S, and SIRC, but these methods are general score fusion methods, while our method is specifically designed for UOSR, so our FS-KNNS surpass them. Our FS-KNNS is totally based on the existing model trained by the classical cross-entropy loss, so there is no extra effort and no outlier data during training, and our FS-KNNS still has better performance than all outlier exposure methods and achieves state-of-the-art UOSR performance, as shown in Fig.~\ref{fig:UOSR_OSR} (b) and~\ref{fig:all_video}. Note that the best choice for OSR (FS-KNN or SSD) may not be the best choice for UOSR (FS-KNNS), as their expectation of InC/InW is contradictory, which shows the necessity of our proposed few-shot UOSR.
% \begin{table}[t]
% \centering
% \tablestyle{1pt}{0.5}
% \caption{Results of few-shot UOSR in the video domain. Model is TSM with pre-training. InD and OoD datasets are UCF101 and HMDB51.}
% \vspace{-3mm}
% \label{tab:fs_video}
% \begin{tabular}{lccccccccccccccc}
% \toprule[1pt]
% &\multicolumn{5}{c}{\bf{5-shot}} &\multicolumn{5}{c}{\bf{1-shot}}\\ \cmidrule(r){2-6} \cmidrule(r){7-11}
% &\bf{AURC$\downarrow$} &  \multicolumn{4}{c}{\bf{AUROC$\uparrow$}} &\bf{AURC$\downarrow$} &  \multicolumn{4}{c}{\bf{AUROC$\uparrow$}}\\ \cmidrule(r){2-2} \cmidrule(r){3-6} \cmidrule(r){7-7} \cmidrule(r){8-11}
% \bf{Methods}  &\bf{UOSR} &\bf{UOSR} & \bf{OSR} &\bf{InC/OoD} &\bf{InC/InW} &\bf{UOSR} &\bf{UOSR} & \bf{OSR} &\bf{InC/OoD} &\bf{InC/InW}\\ \midrule
% SoftMax   &66.05  &93.66 &91.44 &93.46 &\bf{94.99} &66.05  &93.66 &91.44 &93.46 &\bf{94.99}\\
% KNN  &73.73 &93.38 &92.99 &94.11 &88.44 &73.73 &93.38 &92.99 &94.11 &88.44\\ \midrule
% FS-KNN &68.44 &95.04 &\bf{96.14} &\bf{96.71} &83.74 &73.19 &93.60 &\bf{94.32} &95.09 &83.53\\
% SSD &70.36 &93.91 &95.41 &95.97 &79.97 &75.61 &92.48 &93.34 &94.07 &81.75  \\ \midrule
% FS-KNN+S &65.64 &95.44 &94.69 &96.13 &90.78 &68.98 &94.54 &93.66 &95.14 &90.48 \\
% FS-KNN*S &65.29 &94.09 &92.13 &93.96 &\bf{94.99} &65.42 &94.04 &92.08 &93.91 &94.97 \\
% SIRC &62.41 &95.11 &93.79 &95.13 &94.94 &63.11 &94.88 &93.49 &94.88 &94.84 \\ \midrule
% FS-KNNS &\bf{60.43} &\bf{96.25} &95.54 &96.56 &94.14 &\bf{62.65} &\bf{95.35} &94.26 &\bf{95.48} &94.49\\
% \bottomrule[1pt]
% \end{tabular}
% \vspace{-0.3cm}
% \end{table}
\begin{table}[t]
\centering
\tablestyle{1pt}{0.5}
\caption{Results of few-shot UOSR in the video domain. Model is TSM with pre-training. InD and OoD datasets are UCF101 and HMDB51. AUORC (\%) and AURC ($\times10^3$) are reported.}
\vspace{-3mm}
\label{tab:fs_video}
\begin{tabular}{lccccccccccccccc}
\toprule[1pt]
&\multicolumn{5}{c}{\bf{5-shot}} &\multicolumn{5}{c}{\bf{1-shot}}\\ \cmidrule(r){2-6} \cmidrule(r){7-11}
&\bf{AURC$\downarrow$} &  \multicolumn{4}{c}{\bf{AUROC$\uparrow$}} &\bf{AURC$\downarrow$} &  \multicolumn{4}{c}{\bf{AUROC$\uparrow$}}\\ \cmidrule(r){2-2} \cmidrule(r){3-6} \cmidrule(r){7-7} \cmidrule(r){8-11}
\bf{Methods}  &\cellcolor{gray_2}\bf{UOSR} &\cellcolor{gray_2}\bf{UOSR} & \bf{OSR} &\bf{InC/OoD} &\bf{InC/InW} &\cellcolor{gray_2}\bf{UOSR} &\cellcolor{gray_2}\bf{UOSR} & \bf{OSR} &\bf{InC/OoD} &\bf{InC/InW}\\ \midrule
SoftMax   &\cellcolor{gray_2}66.55  &\cellcolor{gray_2}93.66 &91.44 &93.46 &\bf{94.99} &\cellcolor{gray_2}66.55  &\cellcolor{gray_2}93.66 &91.44 &93.46 &\bf{94.99}\\
KNN  &\cellcolor{gray_2}73.73 &\cellcolor{gray_2}93.38 &92.99 &94.11 &88.44 &\cellcolor{gray_2}73.73 &\cellcolor{gray_2}93.38 &92.99 &94.11 &88.44\\ \midrule
FS-KNN &\cellcolor{gray_2}68.44 &\cellcolor{gray_2}95.04 &\bf{96.14} &\bf{96.71} &83.74 &\cellcolor{gray_2}73.19 &\cellcolor{gray_2}93.60 &\bf{94.32} &95.09 &83.53\\
SSD &\cellcolor{gray_2}70.36 &\cellcolor{gray_2}93.91 &95.41 &95.97 &79.97 &\cellcolor{gray_2}75.61 &\cellcolor{gray_2}92.48 &93.34 &94.07 &81.75  \\ \midrule
FS-KNN+S &\cellcolor{gray_2}65.64 &\cellcolor{gray_2}95.44 &94.69 &96.13 &90.78 &\cellcolor{gray_2}68.98 &\cellcolor{gray_2}94.54 &93.66 &95.14 &90.48 \\
FS-KNN*S &\cellcolor{gray_2}65.29 &\cellcolor{gray_2}94.09 &92.13 &93.96 &\bf{94.99} &\cellcolor{gray_2}65.42 &\cellcolor{gray_2}94.04 &92.08 &93.91 &94.97 \\
SIRC &\cellcolor{gray_2}62.41 &\cellcolor{gray_2}95.11 &93.79 &95.13 &94.94 &\cellcolor{gray_2}63.11 &\cellcolor{gray_2}94.88 &93.49 &94.88 &94.84 \\ \midrule
FS-KNNS &\cellcolor{gray_2}\bf{60.00} &\cellcolor{gray_2}\bf{96.19} &95.37 &96.40 &94.82 &\cellcolor{gray_2}\bf{62.65} &\cellcolor{gray_2}\bf{95.35} &94.26 &\bf{95.48} &94.49\\
\bottomrule[1pt]
\end{tabular}
\vspace{-0.3cm}
\end{table}





==> tex/6_conclusion.tex <==
\section{Conclusion}

Rejecting both InW and OoD samples during evaluation has very practical value in most real-world applications, but UOSR is a newly proposed problem and lacks comprehensive analysis and research, so we look deeper into the UOSR problem in this work. We first demonstrate the uncertainty distribution of almost all existing OSR methods is actually closer to the expectation of UOSR than OSR, and then analyze two training settings including pre-training and outlier exposure. Finally, we introduce a new evaluation setting into UOSR, which is few-shot UOSR, and we propose a FS-KNNS method that achieves state-of-the-art performance under all settings.

{\bf Reproducibility Statement}

We provide the uncertainty distribution result files and corresponding codes required to reproduce Tables~\ref{tab:U_OSR_image},~\ref{tab:U_OSR_video},~\ref{tab:bench_r50},~\ref{tab:bench_tsm},~\ref{tab:fs_r50} and~\ref{tab:fs_video} in the supplementary material folder \textit{UOSR/UOSR\_eval}. The users do not need to run the training or evaluation process for a deep learning model. Simply follow the \textit{README\_UOSR\_eval.md} in the \textit{UOSR/UOSR\_eval} folder and all performance results can be printed in the terminal in the table form.

We also provide the training codes for all methods under all settings (pre-training and outlier exposure) based on the ResNet50 backbone in the supplementary material folder \textit{UOSR/UOSR\_train}. The corresponding guideline is in \textit{README\_UOSR\_train.md}. The datasets and experiments details can be found in Appendix~\ref{app:b}.

How to conduct few-shot evaluation to obtain the corresponding uncertainty distribution result files is also included in the supplementary material folder \textit{UOSR/UOSR\_few\_shot}. The corresponding guideline is in \textit{README\_UOSR\_few\_shot.md}. The ablation study of hyper parameters in our FS-KNNS is in Appendix~\ref{app:ablation_fs}.

